VILA: Improving Structured Content Extraction from Scientific PDFs Using Visual Layout Groups

Accurately extracting structured content from PDFs is a critical first step for NLP over scientific papers. Recent work has improved extraction accuracy by incorporating elementary layout information, e.g., each token's 2D position on the page, into language model pretraining. We introduce new methods that explicitly model VIsual LAyout (VILA) groups, i.e., text lines or text blocks, to further improve performance. In our I-VILA approach, we show that simply inserting special tokens denoting layout group boundaries into model inputs can lead to a 1.9% Macro F1 improvement in token classification. In the H-VILA approach, we show that hierarchical encoding of layout-groups can result in up-to 47% inference time reduction with less than 0.8% Macro F1 loss. Unlike prior layout-aware approaches, our methods do not require expensive additional pretraining, only fine-tuning, which we show can reduce training cost by up to 95%. Experiments are conducted on a newly curated evaluation suite, S2-VLUE, that unifies existing automatically-labeled datasets and includes a new dataset of manual annotations covering diverse papers from 19 scientific disciplines. Pre-trained weights, benchmark datasets, and source code are available at https://github.com/allenai/VILA.

==> figures/few-shot.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/few-shot.pdf}
    \caption{Few-shot learning experiments on the \sshard dataset with the ground-truth text block annotations.}
    \label{fig:few-shot}
\end{figure}

==> figures/quadrant.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/quadrant.png}
    \caption{Comparing \vilah and \vilai with Text Blocks and Lines}
    \label{fig:quadrant}
\end{figure}

==> figures/teaser.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/teaser.png}
    \caption{(a) Real-world scientific documents often have intricate layout structures, so analyzing only flattened raw text forfeits valuable information, yielding sub-optimal results. (b) The complex structures can be broken down into groups (text blocks or lines) that are composed of tokens with the same semantic category. (c) We design the \vilai model that injects a special layout indicator token \blk into the text inputs to enable structure-awareness. (d) We also develop a hierarchical model, \vilah, that models each group to reduce the redundant token-level predictions and significantly improve efficiency. Best viewed in color.}
    \label{fig:teaser}
\end{figure*}

==> figures/umap.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/umap.png}
    \caption{UMAP projection of the learned layout contextualized representation for text blocks in H-VILA models}
    \label{fig:umap}
\end{figure}
